Stop Playing the Guessing Game! Target-free User Simulation for Evaluating Conversational Recommender Systems

Recent approaches in Conversational Recommender Systems (CRSs) have tried to simulate real-world users engaging in conversations with CRSs to create more realistic testing environments that reflect the complexity of human-agent dialogue. Despite the significant advancements, reliably evaluating the capability of CRSs to elicit user preferences still faces a significant challenge. Existing evaluation metrics often rely on target-biased user simulators that assume users have predefined preferences, leading to interactions that devolve into simplistic guessing game. These simulators typically guide the CRS toward specific target items based on fixed attributes, limiting the dynamic exploration of user preferences and struggling to capture the evolving nature of real-user interactions. Additionally, current evaluation metrics are predominantly focused on single-turn recall of target items, neglecting the intermediate processes of preference elicitation. To address this, we introduce PEPPER, a novel CRS evaluation protocol with target-free user simulators constructed from real-user interaction histories and reviews. PEPPER enables realistic user-CRS dialogues without falling into simplistic guessing games, allowing users to gradually discover their preferences through enriched interactions, thereby providing a more accurate and reliable assessment of the CRS's ability to elicit personal preferences. Furthermore, PEPPER presents detailed measures for comprehensively evaluating the preference elicitation capabilities of CRSs, encompassing both quantitative and qualitative measures that capture four distinct aspects of the preference elicitation process. Through extensive experiments, we demonstrate the validity of PEPPER as a simulation environment and conduct a thorough analysis of how effectively existing CRSs perform in preference elicitation and recommendation.

==> PEPPER_EMNLP/032rawdataset.tex <==
\begin{table}[ht]
\centering
\caption{Statistics of IMDB user dataset}
\label{tbl:rawdataset}
%\setlength{\tabcolsep}{1mm}{
% \resizebox{0.8\linewidth}{!}
%     {
    \begin{tabular}{lccc}
    \toprule
    \multicolumn{1}{c}{Dataset} & \#Items & \#Users & \#Reviews \\
    \midrule
    {IMDB\textsubscript{Raw}} &{10,116} &{5,000} &{162,067}\\
    \bottomrule
    \end{tabular}
% }
\end{table}


==> PEPPER_EMNLP/040analysis.tex <==
% In this section, we analyze how (1) reliance on target items and (2) use of \text{Recall} as an evaluation metric distort the assessment of CRS performance.

% \input{PEPPER_EMNLP/041biasusertable}
\subsection{How does reliance on target items affect the quality of use-CRS interactions? }
\textbf{Target-biased user simulation results in a guessing game}. \textcolor{red}{As shown in Table ~\ref{tbl:biasresults}, the results reveal a significant performance disparity for target-biased user simulations.
For example, on the IMDB\textsubscript{OpenDialKG} dataset, ChatGPT achieves an average score of 0.874 for the \textit{selected} set but only 0.143 for the \textit{residual} set.
Similar trends are observed in other CRS models and in the results from the IMDB\textsubscript{ReDial} dataset, further confirming the presence of significant bias. 
We interpret this bias as a consequence of target disclosure, where target-biased user simulators tend to prioritize certain target items based on their known attributes, resulting in static and narrowly focused preferences that fail to generalize to the \textit{residual} set.
Moreover, target-biased simulators tend to provide shortcuts for CRSs by explicitly revealing the target item attributes, reducing the need for meaningful preference elicitation and disrupting the natural progression of the recommendation process.}

\subsection{How reliable is Recall as a metric for evaluating CRS in multi-turn dialogues?}
\textbf{Recall suffers from target ambiguity}.
{\color{red}We observe that Recall fails to differentiate whether the CRS is genuinely guiding the conversation toward discovering new target items, or it is simply repeating previously suggested recommendations.
This is clearly illustrated in Figure~\ref{fig:CLR@50}, 
where the results of $\text{Recall}@(t,K)$ exhibit inconsistencies, with the CRSs' performance fluctuating throughout the conversation.}
Notably, we find that \textsc{ChatGPT} exhibits a drop in performance toward the end of the dialogue—even though it generally demonstrates superior context understanding and \textcolor{red}{dialogue shaping} abilities compared to other CRSs.
We speculate that this is because \textsc{ChatGPT}, unlike others, attempts to shift the conversation to elicit new preferences and recommend novel items. However, Recall fails to capture whether these later-turn recommendations are truly new or distinct from previously identified targets, highlighting a key blind spot in its use as an evaluation metric.

\begin{figure}[h]
    \centering
    \includegraphics[width=1\columnwidth]{PEPPER_EMNLP/FIG/PC_Rec_both.pdf}
    \caption{Recall values of the CRSs for every turn $t$ in the IMDB\textsubscript{ReDial} dataset.}
    \label{fig:CLR@50} 
\end{figure}

==> PEPPER_EMNLP/041biasusertable.tex <==
\begin{table}[t]
\centering
\caption{Temp}
\label{tbl:biasuser}
\small
\resizebox{1\linewidth}{!}
{
    \begin{tabular}{cccccc}
    \toprule
    \multirow{2.5}{*}{\textbf{Dataset}} & \multirow{2.5}{*}{\textbf{CRS}} & \multicolumn{4}{c}{\textbf{Target-biased}} \\
     \cmidrule(lr){3-6}
    & & {\textbf{\small PC\textsubscript{selected}@20}} & {\textbf{\small PC\textsubscript{residual}@20}}
    &  {\textbf{\small PC\textsubscript{selected}@50}} & {\textbf{\small PC\textsubscript{residual}@50}} \\
    \midrule 				
    \multirow{4}{*}{IMDB\textsubscript{Redial}}
    &\kbrd 
    & {0.0283} & {0.0158} & {0.0567} & {0.0433} \\
    & \barcor 
     & {0.0667} & {0.0145} & {0.1300} & {0.0517} \\
    &\unicrs 
     & \uline{0.2117} & \textbf{0.0442} & \uline{0.3417} & \uline{0.0658} \\				
    &\chatgpt 
     & \textbf{0.6950} & \uline{0.0267} & \textbf{0.7617} & \textbf{0.0750} \\				
    \midrule   
    \multirow{4}{*}{IMDB\textsubscript{OpenDialKG}}
    &\kbrd 
     & {0.0550} & \uline{0.0433} & {0.1200} & {0.0767} \\							
    &\barcor 
     & {0.1483} & {0.0183} & {0.2033} & {0.0533} \\							
    &\unicrs
     & \uline{0.2233} & {0.0200} & \uline{0.2983} & \uline{0.0900} \\	
    &\chatgpt 
     & \textbf{0.8600} & \textbf{0.1300} & \textbf{0.8950} & \textbf{0.1833} \\
    \bottomrule
    \end{tabular}
}
\end{table}

==> PEPPER_EMNLP/051methodbackup.tex <==
\input{PEPPER_EMNLP/FIG_tex/main_framework}
In this section, we introduce \proposed, a novel evaluation protocol designed to comprehensively assess both preference elicitation and recommendation abilities of CRSs. 
Specifically, it incorporates two key components: (1) target-free user simulators with diverse preferences derived from real user interaction histories and reviews, and (2) preference elicitation metrics that measure a CRS's ability to uncover user preferences and deliver accurate recommendations.

% Task Formulation
% \textbf{Task Formulation.} Given a user-item interaction data, $\mathcal{U}$ and $\mathcal{I}$ denote the set of users and items, respectively.
% The set of user-item interactions and target items are represented by
% \( Z(u)=\{i_u^1, \ldots , i_u^M\} \) and \( Y(u) = \{y_u^1, \ldots, y_u^N\} \), where \( u \in \mathcal{U} \), \( i_u^m \in \mathcal{I}, y_u^n \in \mathcal{I} \), and $M$, $N$ is the number of interactions (i.e., already-interacted items) and target items, respectively.
% The dialogue context $D_t^u = (u_1, r_1, u_2, \ldots, r_t) $ consists of utterances up to t-th turn, $u_t$ and $r_t$ are utterances from the user simulator and CRS, respectively.
% At the t-th turn, the CRS generates an utterance $r_t$ and predicts item list $P_t$
% \begin{equation}
%     r_t, P_t^u = \text{CRS}(D_{t-1}^u, u_t)
% \end{equation} 
% The goal of CRS is to find out target items in $Y(u)$, representing the items that the user $u$ may be interested in, from the entire item set $\mathcal{I}$ through multi-turn natural language conversations.

% Interaction Environment
\subsection{Interaction Environment}
Figure~\ref{fig:overview} illustrates the overall interaction flow of our framework, which comprises two generative agents: a target-free user simulator and a CRS. These agents engage through a dialogue interface and an item interface.
The dialogue interface bridges communication between the user and the CRS, while the item interface presents top-$K$ recommendations predicted by the CRS at each turn, along with their metadata (\textit{i.e.,} movie plots).
By incorporating the item interface, we closely emulate real-world scenarios where users can access detailed information about the recommended items.

For user simulation, we start by extracting the most representative preferences from a user's raw reviews and categorize them into \textit{Likes} and \textit{Dislikes}.
These preferences are then transformed into descriptive narratives, depicting the general preferences of the user simulator.
Next, the user simulator initiates a entirely new conversation by requesting recommendations that align with its general preferences. 
In response, the CRS generates an utterance and presents the top-$K$ item suggestions through the item interface.
As interactions continue, the user simulator not only communicates with the recommender but also engages with the item interface by carefully examining each suggested item. 
For previously interacted items (i.e., seen), it retrieves past reviews, while for newly encountered items (i.e., unseen), it shapes opinions based on its general preferences.
This dual engagement allows the simulator to elicit its own preferences and provide detailed feedback during subsequent interactions, thereby enriching the dialogue to better align with the user's interests and facilitating the discovery of relevant items.

% Target-free User Simulator
\subsection{Target-free User Simulator} \label{sec:targetfree}
Unlike traditional approaches \cite{wang2023rethinking, zhu2024reliable, zhu2025llm, huang2024concept}, which assume scenarios where users have specific preferences about the target items, we design our user simulators with diverse preferences derived from actual user experiences.
We aim to construct target-free simulators, instructing them to seek target items without any predefined target information. Instead, these user simulators gradually elaborate on their preferences through ongoing conversations, mirroring how real users naturally articulate and discover their interests. 
To achieve this, we introduce two core components: \textit{General Preferences} and \textit{Reflected Preferences}.
Specifically, general preferences are established as a foundational profile for the user simulator, providing a broad base of interests and inclinations.
Reflected preferences, on the other hand, enrich the conversation context by allowing the user simulator to dynamically adapt to the interaction, accordingly refine its preferences, and thoughtfully respond to the CRS.

% General Preferences
\subsubsection{General Preferences}\label{sec:general-preferences}
To establish general preferences, we leverage a real-world user database with extensive interaction histories and informative reviews. 
These reviews provide insights into personal preferences that extend beyond simple item attributes, capturing nuanced opinions on aspects such as storyline, pacing, and emotions.
However, since reviews often contain noise and ambiguous expressions, following \cite{kim2024pearl}, we employ ChatGPT to extract and transform each collected reviews into clear, structured binary preferences categorized into \textit{Likes} and \textit{Dislikes}.
{\color{red}We then divide the interaction histories of each user into two distinct sets: \textit{seen} items and \textit{target} items. 
When generating general preferences, we provide ChatGPT with the metadata and corresponding binary preferences of only the \textit{seen} items. 
The model is then instructed to generate descriptive narratives highlighting the most representative features.
These narratives are subsequently used to initialize our user simulators, with each simulator tailored to mimic a distinct instance from the user database.
Through this approach, we ensure that user simulators remain blind to target items while being grounded in detailed general preferences. 
This enables the simulators to possess general preferences that are sufficiently generalizable to discover target preferences, thereby closely emulating real user behaviors.}

% Reflected Preferences
\subsubsection{Reflected Preferences}
\label{subsubsec:PrefRef}
Beyond simply articulating general preferences, real users evaluate items through the lens of their past interactions, preferences, or expectations.
Humans tend to uncover their implicit preferences while interacting with recommendation systems, demonstrating a dynamic and adaptable nature. 
Reflected preference functions to capture this nuanced behavior, enabling user simulators to reflect their preferences with regard to current recommendations responsively. 
{\color{red}To achieve this, we categorize the items presented in the item interface into two sets: a \textit{seen} set and an \textit{unseen} set.
For \textit{seen} items, we allow the user simulators to revisit their corresponding reviews and recalling what they liked or disliked.
For \textit{unseen} items, we prompt the user simulators to shape opinions that align with their general preferences, identifying what they are expected to like or dislike.
These reflected preferences are then provided as additional input for the user’s subsequent response.
This approach enables user simulators to proactively provide feedback on both previously interacted items and newly encountered ones, consequently enriching the dialogue contexts.}

% Evaluation Methodology
\subsection{Evaluation on Preference Elicitation}
\label{subsec:Evaluation}
Since the preference elicitation ability can be defined as \textit{"how proactively a CRS leads the conversation in a natural and engaging manner, guiding the user through discovering a diverse range of preferences to achieve a satisfactory experience"}, 
we consider the following key aspects to evaluate the preference elicitation ability of a CRS.

\begin{itemize}[leftmargin=10pt]

\item \textit{Preference Coverage}: 
evaluates how effectively CRS discover and address the diverse preferences of users through the dialogue.

\item \textit{Proactiveness}~\cite{10.1145/3539618.3594250, deng2024towards}:
characterizes a CRS that actively guides the conversation by making suggestions or asking relevant questions to actively uncover and clarify the user's preferences.

\item \textit{Coherence}~\cite{dziri2019evaluating}:
reflects the CRS's proficiency in maintaining fluid and natural interactions, providing contextually appropriate responses without abrupt transitions or disjointed exchanges.

\item \textit{Personalization}~\cite{lin2023enhancing}: 
refers to how well the system provides recommendations and information that align with the user's preferences, ensuring a satisfying interaction experience.

\end{itemize}
We analyze the preference elicitation capability of CRSs both quantitatively and qualitatively.
For quantitative analysis, we measure \pc to assess how effectively the CRS elicits each user’s preferences with high coverage evolving throughout
the conversation. 
For qualitative analysis, we evaluate Proactiveness, Coherence, and Personalization to assess how effectively the CRS integrates the preference elicitation process into the conversation.

% Quantitative Evaluation Metric
\subsubsection{Quantitative Metric for Preference Elicitation}
To quantitatively measure the system's contextual understanding and recommendation accuracy in the context of conversational continuity, we propose novel metrics, \pc and \pcir.
% While traditional metrics like Recall provide valuable insights, they are not sufficient to fully capture the dynamics of multi-turn interactions.
% Specifically, to evaluate Recall in the context of continuous conversations, we typically note $\text{Recall}@(t, K)$ as the value of Recall@K at the $t$-th turn, reflecting the system's retrieval performance at each interaction. 
% However, this falls short in addressing the success rate~\cite{sun2018conversational, lin2023enhancing, deng2021unified} of retrieving target items that align with diverse user preferences.
% To bridge this gap, we introduce \pc, defined as follows:
%%%%%%%
% We first present a notation for measuring Recall from the perspective of multi-turn interactions.
% To assess Recall in the context of the continuity of conversations, we note $\text{Recall}@(t, K)$ as the value of Recall@K at the t-th turn.
% However, this cannot cover the success rate~\cite{sun2018conversational, lin2023enhancing, deng2021unified} of target items that align with diverse user preferences.
% Therefore, we define a new quantitative metric, \pc for CRS evaluation as follows:
%%%%%%%
{\color{red}Typically, we denote $\text{Recall}@(t, K)$ as the measure for Recall in multi-turn interactions, which captures the value of Recall@K at the $t$-th turn.
While Recall provides valuable insights, it is insufficient for evaluating the success rate~\cite{sun2018conversational, lin2023enhancing, deng2021unified}, particularly in assessing how effectively the system uncovers diverse user preferences as the dialogue progresses.}
To bridge this gap, we introduce \pc, defined as follows:
\begin{equation}
    \label{eq:PC}
    \text{PC}_t = \frac{1}{|U|} \sum_{u \in U} \cfrac{|(\bigcup_{x=1}^t P_x^u) \cap Y(u)|}{|Y(u)|}
\end{equation}
{\color{red}This metric cumulatively measures the capability of a CRS to address diverse user preferences and provide appropriate recommendations.} 

Building on this concept, we define \pcir at round t as follows:
\begin{equation}
    \label{eq:PCIR}
    \textsc{PCIR}_t = \textsc{PC}_{t} - \textsc{PC}_{t-1}
\end{equation}
{\color{red} \textsc{PCIR$_{t}$} indicates the change of \pc between round t-1 and t.
The incremental rate of \textsc{PC} can be interpreted as the extent to which the system discovers new preferences and provides corresponding recommendations at each turn.}
% It can be used to measure the proportion of newly elicited preferences captured by CRS during the conversation.

% \begin{equation}
%     \label{eq:Recall}
%      \text{Recall}_t@K = \frac{1}{|U|} \sum_{u \in U} \cfrac{|P_t^u \cap Y(u)|}{|Y(u)|}
% \end{equation}
% Then we notate $\text{Recall}_1^T@K$ as the average Recall for the entire conversation up to the T-th turn, expressed as follows:
% \begin{equation}
% \label{eq:avgR}
%     \text{Recall}_1^T@K = \frac{1}{T}{\sum_{t=1}^T\text{Recall}_t{@K}}
% \end{equation}

% Qualitative Evaluation
\subsubsection{Qualitative Metric for Preference Elicitation}
To qualitatively analyze the preference elicitation ability of CRSs, following \cite{liu2023g}, we adopt an automated approach, employing an LLM (i.e., GPT-4.0) as the evaluator. 
Our decision to use GPT-4.0 as a judge is grounded in its superior performance over other language models and its demonstrated approximation of human-like judgments ~\cite{gu2024survey, huang2024empirical, chern2024can, zhang2024comprehensive}.
We task the LLM with fine-grained scoring rubrics on a 1-to-5 scale, with clear criteria for each rating. 
The inputs to our qualitative evaluation process comprise generated dialogues and the general preferences unique to each user simulator. 
In assessing \proact and \coh, the LLM is instructed to carefully analyze the full dialogue history, examining how proactively the system discovers user needs while maintaining a fluent conversational tone. 
For \personal, we leverage the LLM to evaluate whether the recommender's responses, including recommendations and explanations, are consistent with the simulator's general preferences. 


==> PEPPER_EMNLP/063itemcase.tex <==
\begin{table}[thbp]
\centering
\caption{An example of reflected preferences generated when 10 items are presented in the item interface (\chatgpt).}
\label{tbl:itemcase}
%\setlength{\tabcolsep}{1mm}{
\resizebox{1\linewidth}{!}
     {
    \begin{tabular}{Y}
    \toprule
    \rowcolor{gray!15} \textbf{Reflected Preferences at turn} \\
    \textbf{Item}: ``\textit{}'': \\
    \textbf{Like}:  \\
    \textbf{Dislike}:  \\
    \ldots \\    

    {\textbf{User: } } \\
    \ldots \\
    \midrule
    \rowcolor{gray!15} \textbf{Reflected Preferences at turn} \\
    \textbf{Item}: ``\textit{}'': \\
    \textbf{Like}:  \\
    \textbf{Dislike}:  \\
    \ldots \\    

    {\textbf{User: } } \\
    \ldots \\
    \midrule
    % . Together the eleven friends plan to rob five Las Vegas casinos in one night. \ldots \\

    \bottomrule
    \end{tabular}
 }
\end{table}


==> PEPPER_EMNLP/064numhistory.tex <==
\begin{table}[t]
\centering
\caption{Recommendation Accuracy of CRS Models with Target-Free User Simulators and different number of Interaction Histories. We assess $PC@_{50}$ for evaluation.}

\label{tbl:ihnumber}
%\setlength{\tabcolsep}{1mm}{
\resizebox{1\linewidth}{!}
    {
    \begin{tabular}{cccccc}
    \toprule
    %\multirow{2.5}{*}{Dataset} 
    & \multirow{2.5}{*}{CRS} & \multicolumn{4}{c}{\# of Interaction Histories} \\
    \cmidrule(lr){3-6}
     & & \text 5 & 10 & 15 & 20 \\
     \midrule 
     \multirow{4}{*}{\rotatebox{90}{\makecell{{IMDB} \\{\textsuperscript{{ReDial}}}}}} &
     
     \kbrd & {0.0200} & {0.0260} & {0.0180} & {0.0160}\\
     
     & \barcor & {0.0640} & {0.05200} & {0.0540} & {0.0480}\\
     
     & \unicrs & \uline{0.0500} & \uline{0.0560} & \uline{0.0560} & \uline{0.0600}\\
     
     & \chatgpt & \textbf{0.0860} & \textbf{0.0860} & \textbf{0.0740} & \textbf{0.0760}\\
     
     \midrule
     \multirow{4}{*}{\rotatebox{90}{\makecell{{IMDB} \\
     {\textsuperscript{{OpenDialKG}}}}}} & 
     
     \kbrd & {0.0920} & {0.1080} & {0.1120} & {0.0920}\\
     
     & \barcor & {0.0900} & {0.1060} & {0.1000} & {0.0978}\\
     
     & \unicrs & \uline{0.1300} & \uline{0.1540} & \uline{0.1440} & \uline{0.1420}\\
     
     & \chatgpt & \textbf{0.1920} & \textbf{0.1920} & \textbf{0.1900} & \textbf{0.1640}\\
     
    \bottomrule
    \end{tabular}
}
\end{table}


==> PEPPER_EMNLP/065biastable.tex <==
\setlength{\tabcolsep}{2pt}   % 기본 6 pt → 2 pt
\renewcommand{\arraystretch}{1.1}
\newcommand{\GradDelta}[1]{#1}  % 임시 정의
\newcolumntype{C}{@{\hspace{3pt}}c@{\hspace{3pt}}}
% ------------------------------------------------------------
%  ❚  TABLE (본문)  ❚
% ------------------------------------------------------------
\begin{table}[h]
\centering
\footnotesize                       % 글자 크기 한 단계 ↓ (보통 \small 이나 \footnotesize)
%
\resizebox{\columnwidth}{!}{        % ★ 한 칼럼 폭에 맞게 스케일링
\begin{tabular}{p{1.2cm} C *{6}{C}} % 1.6 cm 고정폭 + 1 + 6 = 8 칼럼
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{CRS}} &
\multicolumn{3}{c}{\textbf{Target-{biased}}} &
\multicolumn{3}{c}{\textbf{Target-free}} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}
 & & PC$_\mathrm{sel}$ & PC$_\mathrm{res}$ & $\boldsymbol{\Delta}$ &
     PC$_\mathrm{sel}$ & PC$_\mathrm{res}$ & $\boldsymbol{\Delta}$ \\
\midrule
\multirow{4}{*}{\makecell[l]{IMDB\\\textsubscript{Redial}}}
  & KBRD   & 0.040 & 0.030 & \cellcolor{gray!20}\GradDelta{-0.010} & 0.060 & 0.050 & \cellcolor{gray!20}\GradDelta{-0.010} \\
  & BARCOR & 0.285 & 0.165 & \cellcolor{red!10}\GradDelta{-0.120} & 0.135 & 0.160 & \cellcolor{gray!20}\GradDelta{+0.025} \\
  & UniCRS & 0.410 & 0.160 & \cellcolor{red!20}\GradDelta{-0.250} & 0.130 & 0.110 & \cellcolor{gray!20}\GradDelta{-0.020} \\
  & ChatGPT& 0.850 & 0.090 & \cellcolor{red!40}\GradDelta{-0.760} & 0.120 & 0.125 & \cellcolor{gray!20}\GradDelta{+0.005} \\
\midrule
\multirow{4}{*}{\makecell[l]{IMDB\\\textsubscript{OpenDialKG}}}
  & KBRD   & 0.125 & 0.095 & \cellcolor{red!5}\GradDelta{-0.030} & 0.125 & 0.090 & \cellcolor{red!5}\GradDelta{-0.035} \\
  & BARCOR & 0.155 & 0.115 & \cellcolor{red!5}\GradDelta{-0.040} & 0.155 & 0.155 & \cellcolor{gray!20}\GradDelta{+0.000} \\
  & UniCRS & 0.305 & 0.105 & \cellcolor{red!20}\GradDelta{-0.200} & 0.125 & 0.120 & \cellcolor{gray!20}\GradDelta{-0.005} \\
  & ChatGPT& 0.950 & 0.245 & \cellcolor{red!40}\GradDelta{-0.705} & 0.200 & 0.200 & \cellcolor{gray!20}\GradDelta{+0.000} \\
\bottomrule
\end{tabular}}
%
\vspace{-0.3cm}  % 필요하면 캡션 위·아래 여백 조정
\caption{Recommendation Accuracy of CRSs under target-biased and target-free user simulations. We report PC\textsubscript{selected}@50, PC\textsubscript{residual}@50, and their difference (\textbf{$\Delta$}) from 100 randomly sampled user instances.}
\vspace{-0.3cm}
\label{tbl:biasresults}
\end{table}

% \begin{table}[t]
% \centering
% %\setlength{\tabcolsep}{1mm}{
% \resizebox{0.99\linewidth}{!}
% {
%     \begin{tabular}{cccccccccc}
%     \toprule
%     \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{CRS}} & \multicolumn{3}{c}{\textbf{Target-biased}} & \multicolumn{3}{c}{\textbf{Target-free}} \\
%      \cmidrule(lr){3-5} \cmidrule(lr){6-8}
%     & & {\textbf{PC\textsubscript{selected}}} & {\textbf{PC\textsubscript{residual}}}
%     &  {\textbf{$\Delta$}} 
%     & {\textbf{PC\textsubscript{selected}}} & {\textbf{PC\textsubscript{residual}}}
%     &  {\textbf{$\Delta$}}\\
%     \midrule 				
%     \multirow{4}{*}{IMDB\textsubscript{Redial}}
%     &\kbrd 
%     & 0.040 & 0.030 & \GradDelta{-0.010}
%     & 0.060 & 0.050 & \GradDelta{-0.010} \\
%     & \barcor 
%      & 0.285 & 0.165 & \GradDelta{-0.120} 
%      & {0.135} & {0.160} & \GradDelta{+0.025}\\
%     &\unicrs 
%      & {0.410} & {0.160} & \GradDelta{-0.250}
%      & {0.130} & {0.110} & \GradDelta{-0.020} \\				
%     &\chatgpt 
%      & {0.850} & {0.090} & \GradDelta{-0.760} 
%      & 0.120 & {0.125} & \GradDelta{+0.005} \\				
%     \midrule   
%     \multirow{4}{*}{IMDB\textsubscript{OpenDialKG}}
%     &\kbrd 
%      & {0.125} & {0.095} & \GradDelta{-0.030}
%      & {0.125} & 0.090 & \GradDelta{-0.035} \\							
%     &\barcor 
%      & {0.155} & {0.115} & \GradDelta{-0.040}
%      & {0.155} & {0.155} & \GradDelta{+0.000} \\							
%     &\unicrs
%     & {0.305} & {0.105} & \GradDelta{-0.200} 
%     & 0.125   & {0.120} & \GradDelta{-0.005} \\	
    
%     &\chatgpt 
%     & {0.950} & {0.245} & \GradDelta{-0.705}
%     & {0.200} & {0.200} & \GradDelta{+0.000} \\
%     \bottomrule
%     \end{tabular}
% }
% \vspace{-0.2cm}
% \caption{Recommendation Accuracy of CRSs under target-biased and target-free user simulations. We report PC\_selected@50, PC\_residual@50, and their difference (\textbf{$\Delta$}) from 100 randomly sampled user instances.
% }
% % \textit{Selected} refers to the subset of target items used for initializing target-biased user simulators, while \textit{residual} refers to the remaining target items.}
% \label{tbl:biasresults}
% \end{table}




% % 필요 패키지: booktabs, multirow, xcolor (Δ 매크로용)
% \begin{table*}[t]
% \centering
% \small                           % 글자 크기 ↓ (필요하면 \footnotesize 등으로 조정)
% \setlength{\tabcolsep}{2.0pt}    % 열 간격 ↓ (디폴트 6pt → 2.5pt)
% \renewcommand{\arraystretch}{1.15} % 행 높이 살짝 ↑
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{l ccc ccc ccc ccc}
% \toprule
% \multirow{3}{*}{\textbf{CRS}} &
% \multicolumn{6}{c}{\textbf{IMDB\textsubscript{Redial}}} &
% \multicolumn{6}{c}{\textbf{IMDB\textsubscript{OpenDialKG}}} \\[.3ex]
% \cmidrule(lr){2-7}\cmidrule(lr){8-13}
% & \multicolumn{3}{c}{\textit{Target-biased}} &
%   \multicolumn{3}{c}{\textit{Target-free}}  &
%   \multicolumn{3}{c}{\textit{Target-biased}} &
%   \multicolumn{3}{c}{\textit{Target-free}} \\
% \cmidrule(lr){2-4}\cmidrule(lr){5-7}
% \cmidrule(lr){8-10}\cmidrule(lr){11-13}
% & PC\textsubscript{sel} & PC\textsubscript{res} & $\Delta$
% & PC\textsubscript{sel} & PC\textsubscript{res} & $\Delta$
% & PC\textsubscript{sel} & PC\textsubscript{res} & $\Delta$
% & PC\textsubscript{sel} & PC\textsubscript{res} & $\Delta$ \\
% \midrule
% KBRD    & 0.040 & 0.030 & \GradDelta{-0.010} & 0.060 & 0.050 & \GradDelta{-0.010}
%         & 0.125 & 0.095 & \GradDelta{-0.030} & 0.125 & 0.090 & \GradDelta{-0.035} \\
% BARCOR  & 0.285 & 0.165 & \GradDelta{-0.120} & 0.135 & 0.160 & \GradDelta{+0.025}
%         & 0.155 & 0.115 & \GradDelta{-0.040} & 0.155 & 0.155 & \GradDelta{+0.000} \\
% UniCRS  & 0.410 & 0.160 & \GradDelta{-0.250} & 0.130 & 0.110 & \GradDelta{-0.020}
%         & 0.305 & 0.105 & \GradDelta{-0.200} & 0.125 & 0.120 & \GradDelta{-0.005} \\
% ChatGPT & 0.850 & 0.090 & \GradDelta{-0.760} & 0.120 & 0.125 & \GradDelta{+0.005}
%         & 0.950 & 0.245 & \GradDelta{-0.705} & 0.200 & 0.200 & \GradDelta{+0.000} \\
% \bottomrule
% \end{tabular}}
% \vspace{-0.2cm}
% \caption{Recommendation Accuracy of CRSs under target-biased and target-free user simulations. We report PC\_selected@50, PC\_residual@50, and their difference (\textbf{$\Delta$}) from 100 randomly sampled user instances.}
% \label{tbl:biasresults}
% \end{table*}




==> PEPPER_EMNLP/067humanevaltable.tex <==
\begin{table}[ht]
\centering
\small
\begin{tabularx}{\linewidth}{X c}
\toprule
\textbf{Target-free vs. Target-biased} & \textbf{Win Ratio (\%)} \\
\midrule
User Engagement \& Feedback Quality    & 78.3 \\
Preference Diversity                   & 64.7 \\
Dialogue Naturalness \& Coherence     & 79.7 \\
\bottomrule
\end{tabularx}
\caption{Human evaluation on pairwise quality comparison of generated dialogues. We report \proposed's win percentages.}
\label{tbl:humaneval}
\end{table}


==> PEPPER_EMNLP/Tables/pepper_mistral_table.tex <==
\begin{table}[ht]
\centering
%\setlength{\tabcolsep}{1mm}{
\resizebox{0.95\linewidth}{!}
    {
    \begin{tabular}{cccccc}
    \toprule
    %\multirow{2.5}{*}{Dataset} 
    & \multirow{2.5}{*}{\textbf{CRS}} & \multicolumn{4}{c}{\textbf{{PEPPER}{\textsuperscript{Mistral}}}}\\
    \cmidrule(lr){3-6}
     & & {\textbf{\small PC\textsubscript{15}@5}} & {\textbf{\small PC\textsubscript{15}@10}} & {\textbf{\small PC\textsubscript{15}@20}} & {\textbf{\small PC\textsubscript{15}@50}} \\
     
     \midrule
     \multirow{4}{*}{\rotatebox{90}{\makecell{{IMDB} \\
     {\textsuperscript{{OpenDialKG}}}}}} & 
     
     \kbrd & {0.015} & {0.041} & {0.047} & {0.106}\\
     
     & \barcor & {0.011} & {0.024} & {0.059} & {0.136}\\
     
     & \unicrs & 0.035 & {0.052} & {0.091} & {0.173}\\
     
     & \chatgpt & \textbf{{0.079}} & \textbf{{0.118} }& \textbf{{0.156}} & {0.236}\\

    & ChatCRS & {0.056} & {0.069} & {0.127} & {0.231}\\

    & MACRS & {0.044} & {0.074} & {0.129} & \textbf{{0.267}} \\
     
    \bottomrule
    \end{tabular}
}
\caption{Recommendation Accuracy of CRS Models with PEPPER (Mistral-7B-Instruct).}
\label{tbl:mistralsim}
\end{table}


==> PEPPER_EMNLP/prompt_example.tex <==
\begin{table*}[h]
    \small
    \centering
    \begin{tabular} {p{14cm}}
    \toprule
    \textbf{General Preference Construction prompt} \\
    \midrule
\textcolor{teal}{\textbf{[Task Description]}}\\
You are a preference summarizer tasked with extracting key preferences from user profiles. You will receive four types of user information:\\
1. Movies Watched: Titles of the movies the user has watched.\\
2. Genres Watched: Genres of the movies the user has watched.\\
3. Likes: Aspects the user likes about the movies.\\
4. Dislikes: Aspects the user dislikes about the movies.\\
Summarize the user's general preferences by focusing on the most important and representative features.
\\
\\
\textcolor{teal}{\textbf{[Instructions]}}\\
1. Identify and describe what the user generally likes.
\\
2. Identify and describe what the user generally dislikes.
\\
3. Do not mention phrases like "Based on~".
\\
4. Do not provide explanations or reasons for the user's preferences.
\\
\\
\textbf{Movies Watched :} \{seen movies\}
\\
\textbf{Genres Watched :}  \{seen genres\}
\\
\textbf{Likes :} \{likes\}
\\
\textbf{Dislikes :} \{dislikes\}
\\
\bottomrule
    \end{tabular}
    \caption{The Prompt for General Preference Generation.}
    \label{tab:prompt_gp}
\end{table*}



% 
\begin{table*}
    \small
    \centering
    \begin{tabular}{p{14cm}}
    \toprule
    \textbf{Reflected Preference Generation prompt} \\
    \midrule
\textcolor{teal}{\textbf{[Task Description]}}\\
You are a preference summarizer tasked with extracting key preferences from user profiles. You will receive four types of user information:\\
- Movies Watched: Titles of the movies the user has watched.\\
- Genres Watched: Genres of the movies the user has watched.\\
- Likes: Aspects the user likes about the movies.\\
- Dislikes: Aspects the user dislikes about the movies.\\
Summarize the user's general preferences by focusing on the most important and representative features.\\
\\
\textcolor{teal}{\textbf{[Instructions]}}
- For each movie in <seen movies>, express what you liked and disliked based on your previous review and your general preferences.
\\
- For each movie in <unseen movies>, express what aspects of the movie you think you will like and dislike.
\\
- Think about the likes and dislikes from different perspectives.
\\
- Follow the format below to shape your opinion. 
Do not repeat the movie plots; focus solely on your opinion:\\
    <Movie Title> : 'seen' or 'unseen'
\\
    <Like> : list of positive points.
\\
    <Dislike> : list of negative points.
\\
\\
- Keep your points succinct and clear.
\\
- Do not use any personal pronoun.
\\
- Limit your discussion to the four movies provided.
\\
- Do not repeat your general preferences in your response; focus solely on shaping the opinion on the suggestions.
\\
\\
\textbf{Here's your <general preferences> :} \{general preferences\}
\\
\textbf{Here are <seen movies>; they may be empty :} \{seen\}
\\
\textbf{Here are <unseen movies>:} \{unseen\}
\\
\textbf{Below is the conversation history:} \{conversation history\}
\\
\bottomrule
    \end{tabular}
    \caption{The Prompt for Reflected Preference Construction.}
    \label{tab:prompt_gp}
\end{table*}



\begin{table*}
    \small
    \centering
    \begin{tabular}{p{14cm}}
    \toprule
    \textbf{User Simulator prompt} \\
    \midrule
\textcolor{teal}{\textbf{[Task Description]}}\\
You are a User trying to get a movie recommendation that fits your preferences.\\
You will be provived with:\\
    <general preferences> : A detailed description of your movie preferences.\\
    <opinion> : Your likes and dislikes regarding each suggestion in the current recommendation list.\\
Your task is to generate the User's next response.\\
\\
Instructions :\\
1. Start by engaging with the Recommender.\\
2. Regarding both <general preferences> and <opinion> provided:\\
    - Use the <general preferences> to inform your response, expressing your interests and what you’re looking for.\\
    - Incorporate your <opinion> to give feedback on the current recommendations, mentioning what you did and didn’t like.\\
3. If <opinion> is blank, it means recommendations have not yet been provided.\\
4. Keep asking for new recommendations even if you find suggestions that align with your preferences.\\
5. Keep your utterances casual and simple, using daily English.\\
6. Respond in first-person singular.\\
\\
Important points : \\
1. You are role-playing as a User to generate the User's next response.\\
2. Do not express appreciation for the suggestions.\\
3. Do not use phrases such as "Based on~".\\
4. Do not include "User:" in your responses.\\
\\
\textbf{Below is a detailed description of your <general preferences> :}  \{general preferences\}\\
\textbf{Below is your <opinion> about current recommendation list :} \{opinion\} \\
\textbf{Below is the conversation history :}  \{conversation history\}\\
\\
\bottomrule
    \end{tabular}
    \caption{The Prompt for User Simulator instructions.}
    \label{tab:prompt_user}
\end{table*}



\begin{table*}
    \small
    \centering
    \begin{tabular}{p{14cm}}
    \toprule
    \textbf{CRS prompt} \\
    \midrule
\textcolor{teal}{\textbf{[Task Description]}}\\
\textbf{You are a Recommender who recommends a Seeker movies that he/she will enjoy.}\\
\textbf{Follow the instructions below to complete the task:}\\
- Engage with the Seeker to discover his/her movie preferences. \\
- Think about the questions to ask the seeker, and ask the question in your response.\\
- After each interaction, think about whether you have enough information to make a recommendation.\\
- If you think there is enough information, make the recommendation.\\
\\
\bottomrule
    \end{tabular}
    \caption{The Prompt for ChatGPT as zero-shot Conversational Recommender System.}
    \label{tab:prompt_crs}
\end{table*}



\begin{table*}
    \small
    \centering
    \begin{tabular}{p{14cm}}
    \toprule
    \textbf{The Prompt for Qualitative Evaluation on Preference Elicitation Ability of CRS} \\
    \midrule
\textcolor{teal}{\textbf{[Task Description]}}\\
You will be provided with a conversation between a User (annotated as "User") and a Conversational Recommender System (annotated as "Recommender") discussing movie recommendations.\\
Your task is to evaluate and rate the performance of the Conversational Recommender System based on three specific metrics.\\ 
Focus solely on these metrics when assessing each response.\\
Please make sure you read and understand the instructions carefully.\\
\\
\textcolor{teal}{\textbf{[Evaluation Criteria]}}\\
Metric 1 - Proactiveness (1-5): This refers to the system’s capability to take initiative in guiding the conversation, asking relevant questions, and making suggestions to actively uncover and clarify the user’s preferences.\\
1: The Recommender is not proactive.\\
2: The Recommender is slightly proactive.\\
3: The Recommender is moderately proactive.\\
4: The Recommender is mostly proactive.\\
5: The Recommender is completely proactive.\\
\\
Metric 2 - Coherence (1-5): This refers to the system’s capability to engage in fluid interactions with users, providing linguistically natural responses that are contextually related to previous interactions, without abrupt transitions or disjointed exchanges.\\
1: The Recommender's responses are incoherent.\\
2: The Recommender's responses are slightly coherent.\\
3: The Recommender's responses are moderately coherent.\\
4: The Recommender's responses are mostly coherent.\\
5: The Recommender's responses are completely coherent.\\
\\
Metric 3 - Personalization (1-5): This refers to the degree to which the system provides responses that align with the user’s preferences, ensuring a satisfying interaction experience. \\
1: The Recommender does not fulfill the user's preferences. \\
2: The Recommender slightly fulfills the user's preferences. \\
3: The Recommender moderately fulfills the user's preferences. \\
4: The Recommender mostly fulfills the user's preferences. \\
5: The Recommender consistently fulfills the user's preferences. \\
\\
Evaluation Steps :\\
1. Read the entire conversation thoroughly to understand the flow of interaction.\\
2. Rate the CRS’s performance based on the defined metrics (i.e., Proactiveness, Coherence, Personalization) using the 1-5 scale.\\
 \\
Example :\\
\textbf{Conversation History:} \{dialogue history\}\\
\textbf{User preferences:} \{general preferences\} \\
\textbf{You must follow the Evaluation Form below in your response:} Only provide the scores. No explanation is required. \\
- Proactiveness: \\
- Coherence: \\
- Personalization: \\
\\
\bottomrule
    \end{tabular}
    \caption{Qualitative Evaluation Prompt}
    \label{tab:prompt_quali}
\end{table*}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}[h]
%     \small
%     \centering
%     \begin{tabular} {p{14cm}}
%     \toprule
%     \textbf{General Preference Construction prompt} \\
%     \midrule
% \textcolor{teal}{\textbf{[Task Description]}}\\
% You are a preference summarizer tasked with extracting key preferences from user profiles. You will receive four types of user information:\\
% 1. Movies Watched: Titles of the movies the user has watched.\\
% 2. Genres Watched: Genres of the movies the user has watched.\\
% 3. Likes: Aspects the user likes about the movies.\\
% 4. Dislikes: Aspects the user dislikes about the movies.\\
% Summarize the user's general preferences by focusing on the most important and representative features.
% \\
% \\
% Instructions : 
% \\
% 1. Identify and describe what the user generally likes.
% \\
% 2. Identify and describe what the user generally dislikes.
% \\
% 3. Do not mention phrases like "Based on~".
% \\
% 4. Do not provide explanations or reasons for the user's preferences.
% \\
% \\
% \textbf{Movies Watched :} \{seen movies\}
% \\
% \textbf{Genres Watched :}  \{seen genres\}
% \\
% \textbf{Likes :} \{likes\}
% \\
% \textbf{Dislikes :} \{dislikes\}
% \\
% \bottomrule
%     \end{tabular}
%     \caption{The Prompt for General Preference Construction.}
%     \label{tab:prompt_gp}
% \end{table*}



% % 
% \begin{table*}
%     \small
%     \centering
%     \begin{tabular}{p{14cm}}
%     \toprule
%     \textbf{Reflected Preference Construction prompt} \\
%     \midrule
% \textcolor{teal}{\textbf{[Task Description]}}\\
% You are a preference summarizer tasked with extracting key preferences from user profiles. You will receive four types of user information:\\
% 1. Movies Watched: Titles of the movies the user has watched.\\
% 2. Genres Watched: Genres of the movies the user has watched.\\
% 3. Likes: Aspects the user likes about the movies.\\
% 4. Dislikes: Aspects the user dislikes about the movies.\\
% Summarize the user's general preferences by focusing on the most important and representative features.\\
% \\
% Instructions : 
% \\
% 1. For each movie in <seen movies>, express what you liked and disliked based on your previous review and your general preferences.
% \\
% 2. For each movie in <unseen movies>, express what aspects of the movie you think you will like and dislike.
% \\
% 3. Think about the likes and dislikes from different perspectives.
% \\
% 4. Follow the format below to shape your opinion. 
% Do not repeat the movie plots; focus solely on your opinion:\\
% \\
%     <Movie Title> : 'seen' or 'unseen'
% \\
%     <like> : list of positive points
% \\
%     <Dislike> : list of negative points.
% \\
% - Keep your points succinct and clear.
% \\
% - Do not use any personal pronoun.
% \\
% - Limit your discussion to the four movies provided.
% \\
% - Do not remention your general preferences in your response; focus solely on shaping the opinion on the suggestions.
% \\
% \\
% \textbf{Here's your <general preferences> :} \{general preferences\}
% \\
% \textbf{Here are <seen movies>; they may be empty :} \{seen\}
% \\
% \\
% \textbf{Movies Watched :} \{seen movies\}
% \\
% \textbf{Genres Watched :}  \{seen genres\}
% \\
% \textbf{Likes :} \{likes\}
% \\
% \textbf{Dislikes :} \{dislikes\}
% \\
% \bottomrule
%     \end{tabular}
%     \caption{The Prompt for Reflected Preference Construction.}
%     \label{tab:prompt_gp}
% \end{table*}



% \begin{table*}
%     \small
%     \centering
%     \begin{tabular}{p{14cm}}
%     \toprule
%     \textbf{User Simulator prompt} \\
%     \midrule
% \textcolor{teal}{\textbf{[Task Description]}}\\
% You are a User trying to get a movie recommendation that fits your preferences.\\
% You will be provived with:\\
%     <general preferences> : A detailed description of your movie preferences.\\
%     <opinion> : Your likes and dislikes regarding each suggestion in the current recommendation list.\\
% Your task is to generate the User's next response.\\
% \\
% Instructions :\\
% 1. Start by engaging with the Recommender.\\
% 2. Regarding both <general preferences> and <opinion> provided:\\
%     - Use the <general preferences> to inform your response, expressing your interests and what you’re looking for.\\
%     - Incorporate your <opinion> to give feedback on the current recommendations, mentioning what you did and didn’t like.\\
% 3. If <opinion> is blank, it means recommendations have not yet been provided.\\
% 4. Keep asking for new recommendations even if you find suggestions that align with your preferences.\\
% 5. Keep your utterance casual and simple, using daily English.\\
% 6. Respond in first-person singular.\\
% \\
% Important points : \\
% 1. You are role-playing a User to generate User's next response.\\
% 2. Do not express appreciation for the suggestions.\\
% 3. Do not use phrases such as "Based on~".\\
% 4. Do not include "User:" in your responses.\\
% \\
% \textbf{Below is a detailed description of your <general preferences> :}  \{general preferences\}\\
% \textbf{Below is your <opinion> about current recommendation list :} \{opinion\} \\
% \textbf{Below is the conversation history :}  \{conversation history\}\\
% \\
% \bottomrule
%     \end{tabular}
%     \caption{The Prompt for User simulator instructions}
%     \label{tab:prompt_user}
% \end{table*}



% \begin{table*}
%     \small
%     \centering
%     \begin{tabular}{p{14cm}}
%     \toprule
%     \textbf{CRS prompt} \\
%     \midrule
% \textcolor{teal}{\textbf{[Task Description]}}\\
% \textbf{You are a Recommender who recommends a Seeker movies that he/she will enjoy.}\\
% \textbf{Follow the instructions below to complete the task:}\\
% - Engage with the Seeker to discover his/her movie preferences. Think about which question to ask the seeker, and ask the question in your response.\\
% - After each interaction, think about whether you have enough information to make a recommendation.\\
% - If you think there is enough information, make the recommendation.\\
% \\
% \bottomrule
%     \end{tabular}
%     \caption{The Prompt for Conversational Recommender System instructions}
%     \label{tab:prompt_crs}
% \end{table*}



% \begin{table*}
%     \small
%     \centering
%     \begin{tabular}{p{14cm}}
%     \toprule
%     \textbf{The Prompt for Qualitative Evaluation on Preference Elicitation Ability of CRS} \\
%     \midrule
% \textcolor{teal}{\textbf{[Task Description]}}\\
% You will be provided with a conversation between a User (annotated as "User") and a Conversational Recommender System (annotated as "Recommender"), discussing movie recommendations.\\
% Your task is to evaluate and rate the performance of the Conversational Recommender System based on three specific metrics.\\ 
% Focus solely on the metric when assessing each response.\\
% Please make sure you read and understand the instructions carefully.\\
% \\
% Evaluation Crieteria : \\
% Metric 1 - Proactiveness (1-5): This refers to the system’s capability to take initiative in guiding the conversation, asking relevant questions, and making suggestions to actively uncover and clarify the user’s preferences.\\
% 1: The Recommender is not proactive.\\
% 2: The Recommender is slightly proactive.\\
% 3: The Recommender is moderately proactive.\\
% 4: The Recommender is mostly proactive.\\
% 5: The Recommender is completely proactive.\\
% \\
% Metric 2 - Coherence (1-5): this refers to the system’s capability to engage in fluid interactions with users, providing linguistically natural responses that are contextually related to previous interactions, without abrupt transitions or disjointed exchanges.\\
% 1: The Recommender's responses are unnatural.\\
% 2: The Recommender's responses are slightly natural.\\
% 3: The Recommender's responses are moderately natural.\\
% 4: The Recommender's responses are mostly natural.\\
% 5: The Recommender's responses are completely natural.\\
% \\
% Metric 3 - Personalization (1-5): This refers to the degree to which the system provides responses that align with the user’s preferences, ensuring a satisfying interaction experience. \\
% 1: The Recommender doesn't fulfill with the user's preferences. \\
% 2: The Recommender slightly fulfills with the user's preferences. \\
% 3: The Recommender moderately fulfills the user's preferences. \\
% 4: The Recommender mostly fulfills the user's preferences. \\
% 5: The Recommender consistently fulfills the user's preferences. \\
% \\
% Evaluation Steps :\\
% 1. Read the entire conversation thoroughly to understand the flow of interaction.\\
% 2. Rate the CRS’s performance based on the defined metrics (e.g., Proactiveness, Naturalness, Fulfillment) using the 1-5 scale.\\
%  \\
% Example :\\
% \textbf{Conversation History:} \{dialogue history\}\\
% \textbf{User preferences:} \{general preferences\} \\
% \textbf{You must follow the Evaluation Form below in your response:} Only provide the scores, No explanation is required. \\
% - Proactiveness: \\
% - Coherence: \\
% - Fulfillment: \\
% \\
% \bottomrule
%     \end{tabular}
%     \caption{Qualitative Evaluation Prompt}
%     \label{tab:prompt_quali}
% \end{table*}






